Diffusion Large Language Models for Visual Speech Recognition

Existing Visual Speech Recognition (VSR) systems commonly rely on left-to-right autoregressive decoding, which can force premature decisions on visually ambiguous tokens before sufficient context is available. We propose DLLM-VSR, to the best of our knowledge, the first Diffusion Large Language Model (DLLM)-based VSR framework, formulating transcription as iterative masked denoising with flexible-order decoding. With confidence-based unmasking, DLLM-VSR commits high-confidence positions early and uses the committed tokens as bidirectional context to refine ambiguous ones. To adapt DLLMs to VSR, we introduce a two-stage masked-denoising training strategy that separates visual-to-text content alignment from length modeling. We further observe a performance gap compared with an upper-bound setting where the ground-truth transcript length is provided at inference, allowing the model to focus on transcript content decoding. To reduce this gap, we develop length-guided candidate decoding, which uses video duration to construct plausible transcript-length hypotheses and reranks the decoded candidates using length plausibility and decoding confidence. The proposed method achieves a 19.4% word error rate on LRS3, establishing state-of-the-art performance among methods using only LRS3 as labeled training data.

==> table/table6.tex <==
\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.2}
\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{@{}llcccc@{}}
\toprule
\textbf{Encoder} & \textbf{Test Set}
& \textbf{Acc@0} & \textbf{Acc@1} & \textbf{Acc@3} & \textbf{Acc@5} \\
\midrule

\multirow{2}{*}{AV-HuBERT}
& LRS3    & 43.68 & 88.04 & 99.39 & 100.00 \\
& WildVSR & 18.78 & 50.11 & 84.58 & 95.09 \\

\midrule
\multirow{2}{*}{USR~2.0}
& LRS3    & 44.21 & 87.59 & 99.32 & 99.92 \\
& WildVSR & 18.96 & 51.89 & 84.90 & 95.97 \\

\bottomrule
\end{tabular}
\end{adjustbox}
\caption{Length prediction accuracy (\%) across LRS3 and WildVSR using length predictors trained only on LRS3. Acc@$k$ denotes the proportion of test samples whose ground-truth length falls within $\pm k$ tokens of the predicted length.}
\vspace{-2pt}
\label{table:6}
\end{table}
